Computable estimates of the distance to the exact solution of the evolutionary reaction-diffusion equation

We derive guaranteed bounds of distance to the exact solution of the evolutionary reaction-diffusion problem with mixed Dirichlet-Neumann boundary condition. It is shown that two-sided error estimates are directly computable and equivalent to the error. Numerical experiments confirm that estimates provide accurate two-sided bounds of the overall error and generate efficient indicators of local error distribution.

==> customized_packages_and_macros.tex <==
\usepackage[unicode]{hyperref}
\usepackage{amsmath}
\usepackage{graphicx}								% to make \includegraphics work
\usepackage{subfig}
\usepackage{amsfonts} 							% to make \mathbb work
\usepackage{dsfont}
\usepackage{bigints} 								% to use big integrals 
	       														% \bigintssss, \bigintsss, \bigintss, \bigints, and \bigint
\usepackage{algorithm}              % algorithm environment
\usepackage{algorithmic}
\usepackage{booktabs} 							% correct spacing in tables
\usepackage{multirow}								% multirows in tables
\usepackage{setspace}
\usepackage{mathrsfs}
\usepackage[usenames,dvipsnames]{color}



%\usepackage{geometry}
%\geometry{left=2cm}
%\geometry{right=2cm}
%\geometry{top=1cm}
%\geometry{bottom=2cm}


%%--------------------------------------------------------------------------------%%
% to avoid warnings about to big graphics sets
\setlength{\headheight}{32.24043pt}

%%--------------------------------------------------------------------------------%%

\usepackage{tikz}	
\usetikzlibrary{arrows,chains,matrix,positioning,scopes}

\makeatletter
\tikzset{join/.code=\tikzset{after node path={%
\ifx\tikzchainprevious\pgfutil@empty\else(\tikzchainprevious)% 
edge[every join]#1(\tikzchaincurrent)\fi}}}

\makeatother
\tikzset{>=stealth',every on chain/.append style={join}, every join/.style={->}}
\tikzstyle{labeled}=[execute at begin node=$\scriptstyle,   execute at end node=$]

%%--------------------------------------------------------------------------------%%
	
\newcommand {\Int}   {\int\limits}
\newcommand {\Sum}   {\sum\limits}	
\newcommand {\eps}   {\varepsilon}


\newcommand {\IntQT} {\Int_{Q_T}}
\newcommand {\IntTO} {\Int_{t_k}^{t_{k+1}} \Int_\Omega}
\newcommand {\IntTGammaN} {\Int_{t_k}^{t_{k+1}} \Int_{\Gamma_N}}
\newcommand {\IntT}  {\Int_{t_k}^{t_{k+1}}}
\newcommand {\IntO}  {\Int_\Omega}
\newcommand {\IntGammaN}  {\Int_{\Gamma_N}}
\newcommand {\Beta}  {\mathcal{B}}
\newcommand {\waveu} {\widetilde{u}}
\newcommand {\CF}    {C_{\mathrm{F\Omega}}}
\newcommand {\Ctr}   {C_{\mathrm{tr}}}
\newcommand {\Rd}    {{\mathds{R}}^d}
\newcommand {\Rone}  {{\mathds{R}}^1}
\newcommand {\Rtwo}  {{\mathds{R}}^2}
\newcommand {\R}     {\mathscr{R}}
\newcommand {\I}     {\mathscr{I}}
\newcommand {\Ieff}  {{I_{\rm eff}}}
\newcommand {\Ieffmaj}  {{I_{\rm eff}^{\overline{\mathrm M}}}}
\newcommand {\Ieffmin}  {{I_{\rm eff}^{\underline{\mathrm M}}}}
\newcommand {\Ieffmajzero}  {{I_{\rm eff}^{\overline{\mathrm M}_{(0)}}}}
\newcommand {\Ieffmajmuhat}  {{I_{\rm eff}^{\overline{\mathrm M}_{(\hat \mu)}}}}
\newcommand {\Ieffmajone}  {{I_{\rm eff}^{\overline{\mathrm M}_{(1)}}}}

\newcommand*\rfrac[2]{{}^{#1}\!/_{#2}}
\newcommand{\minus}{\scalebox{0.5}[1.0]{\( - \)}}

%%--------------------------------------------------------------------------------%%

\def \NormA#1  {{\mid\mid\mid\! #1 \!\mid\mid\mid}^2 }   % |||...|||
\def \NormAinverse#1  { {\mid\mid\mid\! #1 \!\mid\mid\mid}^2_* }   % |||...|||_*
\def \NormQT#1 {{\mid\!\mid\!\mid #1 \mid\!\mid\!\mid}^2_{Q_T}}   % ||...||
\def \NormQO#1 {{\mid\!\mid\!\mid #1 \mid\!\mid\!\mid}^2_{Q^0}}   % ||...||
\def \NormQk#1 {{\mid\!\mid\!\mid #1 \mid\!\mid\!\mid}^2_{Q^k}}   % ||...||
\def \Normf#1  {\Big \lceil #1 \Big\rceil_\Omega}
\def \dvrg     {\mathrm{div} \:}	
\def \tr       {\mathrm{tr}}
\def \dt       {\mathrm{\:d}t}
\def \dx       {\mathrm{\:d}x}
\def \dxt      {\mathrm{\:d}x\mathrm{d}t}
\def \dst      {\mathrm{\:d}s\mathrm{d}t}
\def \ds       {\mathrm{\:d}s}
\def \Normt#1  {\mid\!\mid\!\mid #1 \mid\!\mid\!\mid}   % |||...|||

% european notation
\def\W#1#2{W^{#1, #2}}
\def\L#1{L^{#1}}
\def\H#1{H^{#1}}
\def\Ho#1{{\mathring{H}}^{#1}}


\def\Maj{\overline{\mathrm M}^2_{(\delta, \, \gamma, \, \mu)}}


\def\Majmu{\overline{\mathrm M}^2_{(\mu )}}
\def\Majmuhat{\overline{\mathrm M}^2_{(\hat \mu )}}
\def\Majone{\overline{\mathrm M}^2_{(1)}}
\def\Majzero{\overline{\mathrm M}^2_{(0)}}

%\def\Maj{{\overline{\mathrm M}^2}}
\def\MajTwo{\overline{\mathrm M}_{(\delta, \gamma, \mu, \epsilon)}}
%\def\MajI#1{\overline{\mathrm M}_{\mathrm{I}}^{#1}}
\def\maj{\overline{\mathrm M}^{2}}
\def\majk#1{\overline{\mathrm M}^{2}_{#1}}
\def\MajII#1{\overline{\mathrm M}_{\mathrm{II}}^{#1}}
\def\Min{{\underline{\mathrm M}^2}}
\def\mink#1{\underline{\mathrm M}^{2}_{#1}}
\def\error{{[e]\,}^2}
\def\mdI{\overline{\mathrm m}^2_{\mathrm{d}}}
\def\mfI{\overline{\mathrm m}^2_{\mathrm{f}}}
\def\Marker{\mathbb M}
\def\bnorm#1{[\!]\,#1\,[\!]}
\def\Indicator{{{ E}\hskip-5.2pt{ I}}\,}
%\def\Rd{\R_d}
%\def\Rf{\R_f}
%\def\Rb{\R_b}

%%--------------------------------------------------------------------------------%%

\newtheorem{thm}{Theorem}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{example}{Example}

\newdefinition{rmk}{Remark}
\newproof{pf}{Proof}
\newproof{pot}{Proof of Theorem \ref{thm2}}

%%--------------------------------------------------------------------------------%%

